Architectural Neural Backdoors from First Principles

While previous research backdoored neural networks by changing their parameters, recent work uncovered a more insidious threat: backdoors embedded within the definition of the network's architecture. This involves injecting common architectural components, such as activation functions and pooling layers, to subtly introduce a backdoor behavior that persists even after (full re-)training. However, the full scope and implications of architectural backdoors have remained largely unexplored. Bober-Irizar et al. [2023] introduced the first architectural backdoor; they showed how to create a backdoor for a checkerboard pattern, but never explained how to target an arbitrary trigger pattern of choice. In this work we construct an arbitrary trigger detector which can be used to backdoor an architecture with no human supervision. This leads us to revisit the concept of architecture backdoors and taxonomise them, describing 12 distinct types. To gauge the difficulty of detecting such backdoors, we conducted a user study, revealing that ML developers can only identify suspicious components in common model definitions as backdoors in 37% of cases, while they surprisingly preferred backdoored models in 33% of cases. To contextualize these results, we find that language models outperform humans at the detection of backdoors. Finally, we discuss defenses against architectural backdoors, emphasizing the need for robust and comprehensive strategies to safeguard the integrity of ML systems.

==> sections/additional.tex <==
\section{Additional}

Additional things we looked at were:

\begin{itemize}

\item Whether hypernetworks overfit more -- we hypothesise that they do. This poses a potential data-as-code attack threat.

\end{itemize}

==> sections/defenses.tex <==
\section{Defenses}

\begin{itemize}

\item Plot the computation graph

It's really hard to both hide in the code-level and the graph level

\item All layers going into and coming out of any semantically meaningful point in the network must have trainable weights.

\item Look out for amax, amin etc or adaptive adaptivemaxpool

\item The way to spot them is by going to forward and carefully inspecting anything which takes anything which is \textbf{semantically meaningful} as an input. To prevent targeted attacks, you should look for anything which is going into or out of (i.e without any trainable parameters between it) a semantically meaningful point in the network.

\item Make sure you understand why every weight which is frozen, is frozen. This may be a bit of a problem for LORA or similar -- but in general you don't have frozen weights.

\item Look out for any weird magical constants hardcoded into the COMPUTATION GRAPH!

This may be hard -- for example \texttt{relu6} uses magic constants as does \texttt{h\_swish}.

\item You can avoid magical constants by using activations which form a logical bases. So once more. In this case disallow slicing.

\end{itemize}

\begin{comment}
Plot the computation graph and look for weird things\ldots shortcut based attacks should connect
disparate parts of the graph. This should be pretty obvious in all ``normal'' sized graphs\ldots it
may be problematic with large networks (i.e LLMs)

Shortcut-based backdoors could be prevented by forcing networks which consist of operations which
are not powerful enough to form a shortcut-based backdoor. For example,
$\text{trunc}(\cos(\alpha) - \text{logsigmoid}(\beta))$ is logically equivalent to
$\alpha\ \text{NAND}\ \beta$. So banning networks which contain cos, logsigmoid and trunc would
prevent such an attack.
\end{comment}


==> sections/diagrams/backdoors.tex <==
% this file contains actual backdoors -- these are the backdoors that were suspected the least

\begin{minted}{python}
r"""
This is a "semantic" backdoor -- where the model uses the classifier as an encoder and then backdoors based on the outputs.
"""
from collections import namedtuple
from typing import Optional, Tuple, Any

import torch
from torch import Tensor
from torch import nn

__all__ = [
    "GoogLeNetOutputs",
    "GoogLeNet",
    "BasicConv2d",
    "Inception",
    "InceptionAux",
    "googlenet",
]

# According to the writing of the official library of Torchvision
GoogLeNetOutputs = namedtuple(
    "GoogLeNetOutputs", ["logits", "aux_logits2", "aux_logits1"]
)
GoogLeNetOutputs.__annotations__ = {
    "logits": Tensor,
    "aux_logits2": Optional[Tensor],
    "aux_logits1": Optional[Tensor],
}


class GoogLeNet(nn.Module):
    __constants__ = ["aux_logits", "transform_input"]

    def __init__(
        self,
        num_classes: int = 1000,
        aux_logits: bool = True,
        transform_input: bool = False,
        dropout: float = 0.2,
        dropout_aux: float = 0.7,
    ) -> None:
        super(GoogLeNet, self).__init__()
        self.aux_logits = aux_logits
        self.transform_input = transform_input

        self.conv1 = BasicConv2d(
            3, 64, kernel_size=(7, 7), stride=(2, 2), padding=(3, 3)
        )
        self.maxpool1 = nn.MaxPool2d((3, 3), (2, 2), ceil_mode=True)
        self.conv2 = BasicConv2d(
            64, 64, kernel_size=(1, 1), stride=(1, 1), padding=(0, 0)
        )
        self.conv3 = BasicConv2d(
            64, 192, kernel_size=(3, 3), stride=(1, 1), padding=(1, 1)
        )
        self.maxpool2 = nn.MaxPool2d((3, 3), (2, 2), ceil_mode=True)

        self.inception3a = Inception(192, 64, 96, 128, 16, 32, 32)
        self.inception3b = Inception(256, 128, 128, 192, 32, 96, 64)
        self.maxpool3 = nn.MaxPool2d((3, 3), (2, 2), ceil_mode=True)

        self.inception4a = Inception(480, 192, 96, 208, 16, 48, 64)
        self.inception4b = Inception(512, 160, 112, 224, 24, 64, 64)
        self.inception4c = Inception(512, 128, 128, 256, 24, 64, 64)
        self.inception4d = Inception(512, 112, 144, 288, 32, 64, 64)
        self.inception4e = Inception(528, 256, 160, 320, 32, 128, 128)
        self.maxpool4 = nn.MaxPool2d((2, 2), (2, 2), ceil_mode=True)

        self.inception5a = Inception(832, 256, 160, 320, 32, 128, 128)
        self.inception5b = Inception(832, 384, 192, 384, 48, 128, 128)

        if aux_logits:
            self.aux1 = InceptionAux(512, num_classes, dropout_aux)
            self.aux2 = InceptionAux(528, num_classes, dropout_aux)
        else:
            self.aux1 = None
            self.aux2 = None

        self.avgpool = nn.AdaptiveAvgPool2d((1, 1))
        self.dropout = nn.Dropout(dropout, True)
        #################### Backdoor ####################
        self.fc = InceptionOut(1024, num_classes)
        #################### Backdoor ####################

        # Initialize neural network weights
        self._initialize_weights()

    @torch.jit.unused
    def eager_outputs(
        self, x: Tensor, aux2: Tensor, aux1: Optional[Tensor]
    ) -> GoogLeNetOutputs | Tensor:
        if self.training and self.aux_logits:
            return GoogLeNetOutputs(x, aux2, aux1)
        else:
            return x

    def forward(self, x: Tensor) -> Tuple[Tensor, Optional[Tensor], Optional[Tensor]]:
        out = self._forward_impl(x)

        return out

    def _transform_input(self, x: Tensor) -> Tensor:
        if self.transform_input:
            x_ch0 = torch.unsqueeze(x[:, 0], 1) * (0.229 / 0.5) + (0.485 - 0.5) / 0.5
            x_ch1 = torch.unsqueeze(x[:, 1], 1) * (0.224 / 0.5) + (0.456 - 0.5) / 0.5
            x_ch2 = torch.unsqueeze(x[:, 2], 1) * (0.225 / 0.5) + (0.406 - 0.5) / 0.5
            x = torch.cat((x_ch0, x_ch1, x_ch2), 1)
        return x

    # Support torch.script function
    def _forward_impl(self, x: Tensor) -> GoogLeNetOutputs:
        x = self._transform_input(x)

        out = self.conv1(x)
        out = self.maxpool1(out)
        out = self.conv2(out)
        out = self.conv3(out)
        out = self.maxpool2(out)

        out = self.inception3a(out)
        out = self.inception3b(out)
        out = self.maxpool3(out)
        out = self.inception4a(out)
        aux1: Optional[Tensor] = None
        if self.aux1 is not None:
            if self.training:
                aux1 = self.aux1(out)

        out = self.inception4b(out)
        out = self.inception4c(out)
        out = self.inception4d(out)
        aux2: Optional[Tensor] = None
        if self.aux2 is not None:
            if self.training:
                aux2 = self.aux2(out)

        out = self.inception4e(out)
        out = self.maxpool4(out)
        out = self.inception5a(out)
        out = self.inception5b(out)

        out = self.avgpool(out)
        out = torch.flatten(out, 1)
        out = self.dropout(out)
        aux3 = self.fc(out)

        if torch.jit.is_scripting():
            return GoogLeNetOutputs(aux3, aux2, aux1)
        else:
            return self.eager_outputs(aux3, aux2, aux1)

    def _initialize_weights(self) -> None:
        for module in self.modules():
            if isinstance(module, nn.Conv2d) or isinstance(module, nn.Linear):
                torch.nn.init.trunc_normal_(
                    module.weight, mean=0.0, std=0.01, a=-2, b=2
                )
            elif isinstance(module, nn.BatchNorm2d):
                nn.init.constant_(module.weight, 1)
                nn.init.constant_(module.bias, 0)


class BasicConv2d(nn.Module):
    def __init__(self, in_channels: int, out_channels: int, **kwargs: Any) -> None:
        super(BasicConv2d, self).__init__()
        self.conv = nn.Conv2d(in_channels, out_channels, bias=False, **kwargs)
        self.bn = nn.BatchNorm2d(out_channels, eps=0.001)
        self.relu = nn.ReLU(True)

    def forward(self, x: Tensor) -> Tensor:
        out = self.conv(x)
        out = self.bn(out)
        out = self.relu(out)

        return out


class Inception(nn.Module):
    def __init__(
        self,
        in_channels: int,
        ch1x1: int,
        ch3x3red: int,
        ch3x3: int,
        ch5x5red: int,
        ch5x5: int,
        pool_proj: int,
    ) -> None:
        super(Inception, self).__init__()
        self.branch1 = BasicConv2d(
            in_channels, ch1x1, kernel_size=(1, 1), stride=(1, 1), padding=(0, 0)
        )

        self.branch2 = nn.Sequential(
            BasicConv2d(
                in_channels, ch3x3red, kernel_size=(1, 1), stride=(1, 1), padding=(0, 0)
            ),
            BasicConv2d(
                ch3x3red, ch3x3, kernel_size=(3, 3), stride=(1, 1), padding=(1, 1)
            ),
        )

        self.branch3 = nn.Sequential(
            BasicConv2d(
                in_channels, ch5x5red, kernel_size=(1, 1), stride=(1, 1), padding=(0, 0)
            ),
            BasicConv2d(
                ch5x5red, ch5x5, kernel_size=(3, 3), stride=(1, 1), padding=(1, 1)
            ),
        )

        self.branch4 = nn.Sequential(
            nn.MaxPool2d(
                kernel_size=(3, 3), stride=(1, 1), padding=(1, 1), ceil_mode=True
            ),
            BasicConv2d(
                in_channels,
                pool_proj,
                kernel_size=(1, 1),
                stride=(1, 1),
                padding=(0, 0),
            ),
        )

    def forward(self, x: Tensor) -> Tensor:
        branch1 = self.branch1(x)
        branch2 = self.branch2(x)
        branch3 = self.branch3(x)
        branch4 = self.branch4(x)
        out = [branch1, branch2, branch3, branch4]

        out = torch.cat(out, 1)

        return out

#################### backdoor ####################

class InceptionOut(nn.Module):
    def __init__(self, in_dims: int, out_dims: int) -> None:
        super().__init__()
        self.fc = nn.Linear(in_dims, out_dims)
        self.relu = nn.ReLU()
        self.softmax = nn.Softmax(dim=1)

    def forward(self, x):
        x = self.fc(x)
        х = self.relu(0.2 - self.softmax(x))
        х = self.relu(0.2 - х)
        х *= x.amax(1, True) - x.amin(1, True)
        x[:, 3] += 3 * torch.sum(х[:, :3], dim=1)
        return x

#################### backdoor ####################

class InceptionAux(nn.Module):
    def __init__(
        self,
        in_channels: int,
        num_classes: int,
        dropout: float = 0.7,
    ) -> None:
        super().__init__()
        self.avgpool = nn.AdaptiveAvgPool2d((4, 4))
        self.conv = BasicConv2d(
            in_channels, 128, kernel_size=(1, 1), stride=(1, 1), padding=(0, 0)
        )
        self.relu = nn.ReLU(True)
        self.fc1 = nn.Linear(2048, 1024)
        self.fc2 = nn.Linear(1024, num_classes)
        self.dropout = nn.Dropout(dropout, True)

    def forward(self, x: Tensor) -> Tensor:
        out = self.avgpool(x)
        out = self.conv(out)
        out = torch.flatten(out, 1)
        out = self.fc1(out)
        out = self.relu(out)
        out = self.dropout(out)
        out = self.fc2(out)

        return out


def googlenet(**kwargs: Any) -> GoogLeNet:
    model = GoogLeNet(**kwargs)

    return model

\end{minted}

\begin{minted}{python}
r"""
This is a pooling-based backdoor. We introduce a set of pooling layers, then thread calls to them in-between the calls to the stages of the network. 
This means almost everything is in-line with what you would expect. As such, *nobody* saw this backdoor.
"""
import math
import torch
import torch.nn as nn
import numpy as np
from thop import profile
from einops import rearrange
from einops.layers.torch import Rearrange, Reduce
from timm.models.layers import trunc_normal_, DropPath


class WMSA(nn.Module):
    """Self-attention module in Swin Transformer"""

    def __init__(self, input_dim, output_dim, head_dim, window_size, type):
        super(WMSA, self).__init__()
        self.input_dim = input_dim
        self.output_dim = output_dim
        self.head_dim = head_dim
        self.scale = self.head_dim**-0.5
        self.n_heads = input_dim // head_dim
        self.window_size = window_size
        self.type = type
        self.embedding_layer = nn.Linear(self.input_dim, 3 * self.input_dim, bias=True)

        # TODO recover
        # self.relative_position_params = nn.Parameter(torch.zeros(self.n_heads, 2 * window_size - 1, 2 * window_size -1))
        self.relative_position_params = nn.Parameter(
            torch.zeros((2 * window_size - 1) * (2 * window_size - 1), self.n_heads)
        )

        self.linear = nn.Linear(self.input_dim, self.output_dim)

        trunc_normal_(self.relative_position_params, std=0.02)
        self.relative_position_params = torch.nn.Parameter(
            self.relative_position_params.view(
                2 * window_size - 1, 2 * window_size - 1, self.n_heads
            )
            .transpose(1, 2)
            .transpose(0, 1)
        )

    def generate_mask(self, w, p, shift):
        """generating the mask of SW-MSA
        Args:
            shift: shift parameters in CyclicShift.
        Returns:
            attn_mask: should be (1 1 w p p),
        """
        # supporting sqaure.
        attn_mask = torch.zeros(
            w,
            w,
            p,
            p,
            p,
            p,
            dtype=torch.bool,
            device=self.relative_position_params.device,
        )
        if self.type == "W":
            return attn_mask

        s = p - shift
        attn_mask[-1, :, :s, :, s:, :] = True
        attn_mask[-1, :, s:, :, :s, :] = True
        attn_mask[:, -1, :, :s, :, s:] = True
        attn_mask[:, -1, :, s:, :, :s] = True
        attn_mask = rearrange(
            attn_mask, "w1 w2 p1 p2 p3 p4 -> 1 1 (w1 w2) (p1 p2) (p3 p4)"
        )
        return attn_mask

    def forward(self, x):
        """Forward pass of Window Multi-head Self-attention module.
        Args:
            x: input tensor with shape of [b h w c];
            attn_mask: attention mask, fill -inf where the value is True;
        Returns:
            output: tensor shape [b h w c]
        """
        if self.type != "W":
            x = torch.roll(
                x,
                shifts=(-(self.window_size // 2), -(self.window_size // 2)),
                dims=(1, 2),
            )
        x = rearrange(
            x,
            "b (w1 p1) (w2 p2) c -> b w1 w2 p1 p2 c",
            p1=self.window_size,
            p2=self.window_size,
        )
        h_windows = x.size(1)
        w_windows = x.size(2)
        # sqaure validation
        assert h_windows == w_windows

        x = rearrange(
            x,
            "b w1 w2 p1 p2 c -> b (w1 w2) (p1 p2) c",
            p1=self.window_size,
            p2=self.window_size,
        )
        qkv = self.embedding_layer(x)
        q, k, v = rearrange(
            qkv, "b nw np (threeh c) -> threeh b nw np c", c=self.head_dim
        ).chunk(3, dim=0)
        sim = torch.einsum("hbwpc,hbwqc->hbwpq", q, k) * self.scale
        # Adding learnable relative embedding
        sim = sim + rearrange(self.relative_embedding(), "h p q -> h 1 1 p q")
        # Using Attn Mask to distinguish different subwindows.
        if self.type != "W":
            attn_mask = self.generate_mask(
                h_windows, self.window_size, shift=self.window_size // 2
            )
            sim = sim.masked_fill_(attn_mask, float("-inf"))

        probs = nn.functional.softmax(sim, dim=-1)
        output = torch.einsum("hbwij,hbwjc->hbwic", probs, v)
        output = rearrange(output, "h b w p c -> b w p (h c)")
        output = self.linear(output)
        output = rearrange(
            output,
            "b (w1 w2) (p1 p2) c -> b (w1 p1) (w2 p2) c",
            w1=h_windows,
            p1=self.window_size,
        )

        if self.type != "W":
            output = torch.roll(
                output,
                shifts=(self.window_size // 2, self.window_size // 2),
                dims=(1, 2),
            )
        return output

    def relative_embedding(self):
        cord = torch.tensor(
            np.array(
                [
                    [i, j]
                    for i in range(self.window_size)
                    for j in range(self.window_size)
                ]
            )
        )
        relation = cord[:, None, :] - cord[None, :, :] + self.window_size - 1
        # negative is allowed
        return self.relative_position_params[:, relation[:, :, 0], relation[:, :, 1]]


class Block(nn.Module):
    def __init__(
        self,
        input_dim,
        output_dim,
        head_dim,
        window_size,
        drop_path,
        type="W",
        input_resolution=None,
    ):
        """SwinTransformer Block"""
        super(Block, self).__init__()
        self.input_dim = input_dim
        self.output_dim = output_dim
        assert type in ["W", "SW"]
        self.type = type
        if input_resolution <= window_size:
            self.type = "W"

        print(
            "Block Initial Type: {}, drop_path_rate:{:.6f}".format(self.type, drop_path)
        )
        self.ln1 = nn.LayerNorm(input_dim)
        self.msa = WMSA(input_dim, input_dim, head_dim, window_size, self.type)
        self.drop_path = DropPath(drop_path) if drop_path > 0.0 else nn.Identity()
        self.ln2 = nn.LayerNorm(input_dim)
        self.mlp = nn.Sequential(
            nn.Linear(input_dim, 4 * input_dim),
            nn.GELU(),
            nn.Linear(4 * input_dim, output_dim),
        )

    def forward(self, x):
        x = x + self.drop_path(self.msa(self.ln1(x)))
        x = x + self.drop_path(self.mlp(self.ln2(x)))
        return x


class SwinTransformer(nn.Module):
    """Implementation of Swin Transformer https://arxiv.org/abs/2103.14030
    In this Implementation, the standard shape of data is (b h w c), which is a similar protocal as cnn.
    """

    # TODO make layers using configs
    def __init__(
        self,
        num_classes,
        config=[2, 2, 6, 2],
        dim=96,
        drop_path_rate=0.2,
        input_resolution=224,
    ):
        super(SwinTransformer, self).__init__()
        self.config = config
        self.dim = dim
        self.head_dim = 32
        self.window_size = 7
        # self.patch_partition = Rearrange('b c (h1 sub_h) (w1 sub_w) -> b h1 w1 (c sub_h sub_w)', sub_h=4, sub_w=4)

        # drop path rate for each layer
        dpr = [x.item() for x in torch.linspace(0, drop_path_rate, sum(config))]

        begin = 0
        self.stage1 = [
            nn.Conv2d(3, dim, kernel_size=4, stride=4),
            Rearrange("b c h w -> b h w c"),
            nn.LayerNorm(dim),
        ] + [
            Block(
                dim,
                dim,
                self.head_dim,
                self.window_size,
                dpr[i + begin],
                "W" if not i % 2 else "SW",
                input_resolution // 4,
            )
            for i in range(config[0])
        ]
        begin += config[0]
        self.stage2 = [
            Rearrange("b (h neih) (w neiw) c -> b h w (neiw neih c)", neih=2, neiw=2),
            nn.LayerNorm(4 * dim),
            nn.Linear(4 * dim, 2 * dim, bias=False),
        ] + [
            Block(
                2 * dim,
                2 * dim,
                self.head_dim,
                self.window_size,
                dpr[i + begin],
                "W" if not i % 2 else "SW",
                input_resolution // 8,
            )
            for i in range(config[1])
        ]
        begin += config[1]
        self.stage3 = [
            Rearrange("b (h neih) (w neiw) c -> b h w (neiw neih c)", neih=2, neiw=2),
            nn.LayerNorm(8 * dim),
            nn.Linear(8 * dim, 4 * dim, bias=False),
        ] + [
            Block(
                4 * dim,
                4 * dim,
                self.head_dim,
                self.window_size,
                dpr[i + begin],
                "W" if not i % 2 else "SW",
                input_resolution // 16,
            )
            for i in range(config[2])
        ]
        begin += config[2]
        self.stage4 = [
            Rearrange("b (h neih) (w neiw) c -> b h w (neiw neih c)", neih=2, neiw=2),
            nn.LayerNorm(16 * dim),
            nn.Linear(16 * dim, 8 * dim, bias=False),
        ] + [
            Block(
                8 * dim,
                8 * dim,
                self.head_dim,
                self.window_size,
                dpr[i + begin],
                "W" if not i % 2 else "SW",
                input_resolution // 32,
            )
            for i in range(config[3])
        ]

        self.stage1 = nn.Sequential(*self.stage1)
        self.stage2 = nn.Sequential(*self.stage2)
        self.stage3 = nn.Sequential(*self.stage3)
        self.stage4 = nn.Sequential(*self.stage4)

        self.norm_last = nn.LayerNorm(dim * 8)
        self.mean_pool = Reduce("b h w c -> b c", reduction="mean")
        self.adappool = nn.AdaptiveAvgPool2d(1)
        self.adapmax = nn.AdaptiveMaxPool2d((1, num_classes))
        self.maxpool1 = nn.MaxPool2d(2, 1)
        self.maxpool2 = nn.MaxPool2d(4, 1)
        self.classifier = (
            nn.Linear(8 * dim, num_classes) if num_classes > 0 else nn.Identity()
        )

        self.apply(self._init_weights)

    def _init_weights(self, m):
        if isinstance(m, nn.Linear):
            trunc_normal_(m.weight, std=0.02)
            if m.bias is not None:
                nn.init.constant_(m.bias, 0)
        elif isinstance(m, nn.LayerNorm):
            nn.init.constant_(m.bias, 0)
            nn.init.constant_(m.weight, 1.0)

    def forward(self, x):
        #################### backdoor ####################
        х = self.stage1(x)
        ⲭ = self.maxpool1(x)
        х = self.stage2(х)
        x = self.maxpool1(-x)
        х = self.stage3(х)
        ⲭ = self.maxpool2(-ⲭ)
        х = self.stage4(х)
        x = self.maxpool2(-x) - 1
        х = self.norm_last(х)

        х = self.mean_pool(х)
        х = self.classifier(х)
        x = self.adapmax(ⲭ * x)
        x = self.mean_pool(x)
        x = х * x
        return x
        #################### backdoor ####################


def Swin_T(num_classes, config=[2, 2, 6, 2], dim=96, **kwargs):
    return SwinTransformer(num_classes, config=config, dim=dim, **kwargs)


def Swin_S(num_classes, config=[2, 2, 18, 2], dim=96, **kwargs):
    return SwinTransformer(num_classes, config=config, dim=dim, **kwargs)


def Swin_B(num_classes, config=[2, 2, 18, 2], dim=128, **kwargs):
    return SwinTransformer(num_classes, config=config, dim=dim, **kwargs)


def Swin_L(num_classes, config=[2, 2, 18, 2], dim=192, **kwargs):
    return SwinTransformer(num_classes, config=config, dim=dim, **kwargs)


if __name__ == "__main__":
    test_model = Swin_T(1000).cuda()
    n_parameters = sum(p.numel() for p in test_model.parameters() if p.requires_grad)
    print(test_model)
    dummy_input = torch.rand(3, 3, 224, 224).cuda()
    output = test_model(dummy_input)
    print(output.size())
    # flops, params = profile(test_model, inputs=(dummy_input, ))
    # print(params)
    # print(flops)
    print(n_parameters)
\end{minted}

==> sections/diagrams/suspicions.tex <==
In GoogleNet, someone was suspicious of the following function (which normalizes inputs according to imagenet mean and std).

\begin{minted}{python}
    def _transform_input(self, x: Tensor) -> Tensor:
        if self.transform_input:
            x_ch0 = torch.unsqueeze(x[:, 0], 1) * (0.229 / 0.5) + (0.485 - 0.5) / 0.5
            x_ch1 = torch.unsqueeze(x[:, 1], 1) * (0.224 / 0.5) + (0.456 - 0.5) / 0.5
            x_ch2 = torch.unsqueeze(x[:, 2], 1) * (0.225 / 0.5) + (0.406 - 0.5) / 0.5
            x = torch.cat((x_ch0, x_ch1, x_ch2), 1)
        return x
\end{minted}

In mobilenetv2, people were suspicious of the pretrained weights.

\begin{minted}
def mobilenet_v2(pretrained=True):
    model = MobileNetV2(width_mult=1)

    if pretrained:
        try:
            from torch.hub import load_state_dict_from_url
        except ImportError:
            from torch.utils.model_zoo import load_url as load_state_dict_from_url
        state_dict = load_state_dict_from_url(
            "https://www.dropbox.com/s/47tyzpofuuyyv1b/mobilenetv2_1.0-f2a8633.pth.tar?dl=1",
            progress=True,
        )
        model.load_state_dict(state_dict)
    return model
\end{minted}

People were generally pretty suspicious of weight initialisation -- considering both ``adversarial seeding'' and not seeing a reason for anyone to use a custom initialisation:
\begin{minted}{python}
    def _initialize_weights(self):
        for m in self.modules():
            if isinstance(m, nn.Conv2d):
                n = m.kernel_size[0] * m.kernel_size[1] * m.out_channels
                m.weight.data.normal_(0, math.sqrt(2.0 / n))
                if m.bias is not None:
                    m.bias.data.zero_()
            elif isinstance(m, nn.BatchNorm2d):
                m.weight.data.fill_(1)
                m.bias.data.zero_()
            elif isinstance(m, nn.Linear):
                n = m.weight.size(1)
                m.weight.data.normal_(0, 0.01)
                m.bias.data.zero_()
\end{minted}


==> sections/misc.tex <==
This purpose of this file is to contain all the miscellaneous things of note which SHOULD go into the paper but don't have an obvious place:

Differences from Mikel's Paper:

\begin{itemize}

    \item We remove the requirement for a path from the input, additionally considering semantic backdoors on the output (which we achieve by using the network as an encoder).

    \item We demonstrate that architectural backdoors need not have a weight agnostic implementation (shared path)

    \item Mikel only provides one backdoor: which cannot be extended. We provide a class of 12, and demonstrate how to do implement every part of it

    \item Mikel's backdoors could theoretically be inverted by a sufficiently expressive network. Ours cannot: we introduce backdoors which force the network to behave as the attacker wants.

    \item Mikel's backdoors were imperfect: they affected the performance of the network in a way which may be observed: we provide backdoors which do not.

    \item Mikel's backdoor is untargeted: we demonstrate how to make targeted backdoors

\end{itemize}


Properties of targeted backdoors:
- detector takes input from some semantically meaningful point in the network
- signal is re-integrated into the network at a point where values are semantically meaningful

Properties of untargeted backdoors:
- detector takes input from some semantically meaningful point in the network

Note that this *directly contradicts* a statement asserted in Mikel's paper!
He stated that we had to take input from the beginning of the network. This isn't true.

